Noise-tolerant fair classification

Fairness-aware learning involves designing algorithms that do not discriminate with respect to some sensitive feature (e.g., race or gender). Existing work on the problem operates under the assumption that the sensitive feature available in one's training sample is perfectly reliable. This assumption may be violated in many real-world cases: for example, respondents to a survey may choose to conceal or obfuscate their group identity out of fear of potential discrimination. This poses the question of whether one can still learn fair classifiers given noisy sensitive features. In this paper, we answer the question in the affirmative: we show that if one measures fairness using the mean-difference score, and sensitive features are subject to noise from the mutually contaminated learning model, then owing to a simple identity we only need to change the desired fairness-tolerance. The requisite tolerance can be estimated by leveraging existing noise-rate estimators from the label noise literature. We finally show that our procedure is empirically effective on two case-studies involving sensitive feature censoring.

==> Fairness under corruption NeurIPS 2019 (2)/7experiment.tex <==
%auto-ignore
%We present experimental results validating the preceding theory.
%Specifically,
We demonstrate that it is viable to learn fair classifiers given noisy sensitive features.\footnote{\FINALCHANGE{}{Source code is available at \url{https://github.com/AIasd/noise\_fairlearn}.}}
%We present two case studies in which we show that using our method, we can preserve fairness even when data is corrupted.
As our underlying fairness-aware classifier,
we use a modified version of the classifier implemented in \citet{reduction} with the DDP and DEO constraints which, as discussed in \S\ref{section:fairnessdef}, are special cases 
of our more general constraints \eqref{eqn:ddp} and \eqref{eqn:deo}. The classifier's original constraints can also be shown to be noise-invariant but in a slightly different way (see Appendix \ref{appendix:agarwal_constraint} for a discussion). An advantage of this classifier is that it is shown to reach levels of fairness violation that are very close to the desired level ($\tau$), i.e., for small enough values of $\tau$ it will reach the constraint boundary.

While we had to choose a particular classifier, our method can be used before using any downstream fair classifier as long as it can take in a parameter $\tau$ that controls the strictness of the fairness constraint and that its constraints are special cases of our very general constraints \eqref{eqn:ddp} and \eqref{eqn:deo}.

\subsection{Noise setting}
\label{ssec:CCN_and_MC}
% While our results apply for any instantiation of the MC learning noise framework, in practice this general kind of noise is rarely observed.
% Instead, 
Our case studies focus on two common special cases of MC learning: CCN and PU learning.
Under CCN noise the sensitive feature's value is randomly flipped with probability $\rho^+$ if its value was 1, or with probability $\rho^-$ if its value was 0. As shown in \citet[Appendix C]{corruption}, CCN noise is a special case of MC learning. 
% with:
% \begin{align*}
%     \pi_{a,\mathrm{corr}} &= (1-\rho^+) \cdot \pi_{a}+\rho^- \cdot (1-\pi_{a})\\
%     \alpha &= \pi_{a,\text{corr}}^{-1} \cdot (1-\pi_{a}) \cdot \rho^-\\
%     \beta &= (1-\pi_{a,\text{corr}})^{-1} \cdot \pi_{a} \cdot \rho^+
% \end{align*}
For PU learning we consider the censoring setting~\citep{Elkan} which is a special case of CCN learning where one of $\rho^+$ and $\rho^-$ is 0.
While our results also apply to the case-controlled setting of PU learning~\citep{Ward:2009}, the former setting is more natural in our context. Note that from $\rho^+$ and $\rho^-$ one can obtain $\alpha$ and $\beta$ as described in~\citet{corruption}.
%Consequently, in both case studies we only need to estimate $\rho^+$ and $\rho^-$ (as well as $\pi_{a, \text{corr}}$, which is trivial) to be able to calculate the scaling coefficient $1-\alpha-\beta$. Since noise parameter estimation is not the aim of our paper, we assume that
%the values of $\rho^+$ and $\rho^-$ are known.

\subsection{Benchmarks}
% \input{experiment_sanity_check.text}

For each case study, we evaluate our method
(termed {\sf cor scale});
recall this scales the input parameter $\tau$ using Theorem \ref{thm: sensitive noise reduction} and the values of $\rho^+$ and $\rho^-$, and then uses the fair classifier to perform classification.
We compare our method with three  different baselines.
The first two trivial baselines are applying the fair classifier directly on the non-corrupted data (termed {\sf nocor}) and on the corrupted data (termed {\sf cor}). While the first baseline is clearly the ideal, it won't be possible when only the corrupted data is available. The second baseline should show that there is indeed an empirical need to deal with the noise in some way and that it cannot simply be ignored.

% AKM: we do better than denoise
The third, non-trivial, baseline (termed {\sf denoise}) is to first denoise $A$ and then apply the fair classifier on the denoised distribution. This denoising is done by applying the {\sf RankPrune} method in \cite{northcutt2017rankpruning}. Note that we provide {\sf RankPrune} with the same known values of $\rho^+$ and $\rho^-$ that we use to apply our scaling so this is a fair comparison to our method.
%\aditya{Reword ``privacy''.}
{Compared to {\sf denoise}, we do \emph{not} explicitly infer individual sensitive feature values;
thus, our method does not compromise privacy.}

For both case studies, we study the relationship between the input parameter $\tau$ and the testing error and fairness violation. %for all three benchmarks and our method.
For simplicity, we only consider the DP constraint.

%
\subsection{Case study: privacy preservation}\label{casestudy: privacy}
\input{case_study_privacy.tex}


%
\subsection{Case study: PU learning}\label{casestudy: pu}
\input{case_study_pu.tex}


==> Fairness under corruption NeurIPS 2019 (2)/abstract.tex <==
%auto-ignore
%Fair machine learning concerns the analysis and design of learning algorithms that do not exhibit systematic bias with respect to some sensitive feature (e.g., race, gender).
%This subject
% Fair machine learning has %received sustained interest in the past few years, with
% seen considerable progress on both devising sensible measures of fairness, and means of achieving them.
% Typically, the latter
Fairness-aware learning involves designing algorithms that do not discriminate with respect to some sensitive feature (e.g., race or gender). 
Existing work on the problem operates under the assumption that the sensitive feature available in one's training sample is perfectly reliable.
This assumption may be violated in many real-world cases:
for example, respondents to a survey may choose to conceal or obfuscate their group identity out of fear of potential discrimination. 
This poses the question of whether one can still learn fair classifiers given \emph{noisy} sensitive features.
In this paper, we answer the question in the affirmative:
we show that if one measures fairness using the \emph{mean-difference score},
and sensitive features are
subject to noise from
the \emph{mutually contaminated learning} model,
then owing to a simple identity
we only need to change the desired fairness-tolerance.
The requisite tolerance can be estimated by leveraging existing noise-rate estimators from the label noise literature.
%\AKMEDIT{from the label noise literature}.
We finally show that our procedure is empirically effective on two case-studies involving sensitive feature censoring.


==> Fairness under corruption NeurIPS 2019 (2)/background.tex <==
We recall the settings of standard and fairness-aware binary classification%
\footnote{For simplicity, we consider the setting of binary target and sensitive features.
However, our derivation and method can be easily extended to the multi-class setting.},
and establish notation.
%used in the sequel.

Our notation is summarized in Table \ref{table:notation}.

%
\subsection{Standard binary classification}

Binary classification concerns predicting the label or \emph{target feature} $Y \in \set{0,1}$ that best corresponds to a given instance $X \in \cX$.
Formally, suppose $D$ is a distribution over (instance, target feature) pairs from $\cX \times \set{0,1}$.
Let $f \colon \cX \to \R$ be a score function,
and $\cF \subset \R^{\cX}$ be a user-defined class of such score functions.
Finally, let $\ellc: \R \times \set{0,1} \to \R_+$ be a loss function measuring the disagreement between a given score and binary label.
%Without loss of generality we suppose that the classification is done via taking the sign of a score function $f: \R^d \to \R$.
%And:
%$$\Lc_D(f) := \Ex_{(x, a, y) \sim D}[\ellc(f(x), y)]$$
The goal of binary classification is to minimise %$f^*$, where
\begin{align}
    \label{eqn:standard-risk}
    % f^*    &:= \argmin_{f\in \mathcal{F}} \Lc_D(f) \\
    \Lc_D(f) &:= \Ex_{(X, Y) \sim D}[\ellc(f(X), Y)].
\end{align}
% In practice, one only observes samples from $D$, and minimizes the empirical counterpart to $\Lc_D$.

%
\subsection{Fairness-aware classification}
\label{section:fairnessdef}

In fairness-aware classification, the goal of accurately predicting the target feature $Y$ remains.
However, there is an additional \emph{sensitive feature} $A \in \set{0,1}$ upon which we do not wish to discriminate.
Intuitively, some user-defined fairness loss should be roughly the same regardless of $A$.

Formally, suppose $D$ is a distribution over 
(instance, sensitive feature, target feature) triplets from
$\cX \times \{0,1\} \times \{0,1\}$.
%where when $(X,A,Y) \sim D$ we have that $X$ is the feature vector, $A$ is the sensitive attribute, and $Y$ is the label.
%The goal in fair machine learning is to learn a good classifier while keeping unfairness low.
%In fair binary classification, the problem can be formulated as finding $f^*$ where
The goal of \emph{fairness-aware} binary classification is to find%
\footnote{Here, $f$ is assumed to not be allowed to use $A$ at test time, which is a common legal restriction~\citep{lipton2018does}.
Of course, $A$ can be used at training time to find an $f$ which satisfies the constraint.}
%$f^*$, where
\begin{equation}
    \label{eqn:fairness-objective}
    \begin{aligned}
        %f^* := \argmin_{f\in \mathcal{F}} \Lc_D(f) \textrm{ s.t. some fairness constraint(s) }
        f^*    &:= \argmin_{f\in \mathcal{F}} \Lc_D(f), \textrm{ such that } \Lambda_D( f ) \leq \tau \\
        \Lc_D(f) &:= \Ex_{(X, A, Y) \sim D}[\ellc(f(X), Y)],
    \end{aligned}
\end{equation}
for user-specified 
\emph{fairness tolerance} $\tau \geq 0$, and
\emph{fairness constraint} $\Lambda_D \colon \cF \to \R_+$. %is a user-specified the fairness constraint(s) are as described in section \ref{section:fairnessdef}.
Such constrained {optimisation} problems can  be solved in various ways,
e.g., convex relaxations~\citep{Donini:2018},
alternating {minimisation}~\citep{ZafarWWW,Cotter:2018},
or {linearisation}~\citep{Hardt2016}.
% or by 
% considering randomized classifiers to linearize the constraints~\citep{Hardt2016,cost}.

%this definition does not allow $A$ to be used for classification.
% While it would be interesting to extend the approach to when $A$ is available as input to $f$ as well, this proves challenging when subsequently considering the effect of noise on $A$.
%as the noise would then also come into the classifier.

%
%\subsection{Common Group Fairness Definitions}\label{section:fairnessdef}

A number of fairness constraints $\Lambda_D( \cdot )$ have been proposed in the literature.
We focus on two {important and} specific choices in this paper, inspired by~\citet{Donini:2018}:
\begin{align}
    \label{eqn:ddp}
    %&\textbf{DDP}_{\ellf}: 
    \Lambda^{\mathrm{DP}}_D( f ) &:= \abs{ \Lf_{D_{0, \cdot}}(f) - \Lf_{D_{1, \cdot}}(f) } \\ 
    %\leq \tau \\
    %&\textbf{DEO}_{\ellf}: 
    \label{eqn:deo}
    \Lambda^{\mathrm{EO}}_D( f ) &:= \abs{ \Lf_{D_{0, 1}}(f) - \Lf_{D_{1, 1}}(f) }, 
    %\leq \tau,
\end{align}
where we denote by $D_{a,\cdot},D_{\cdot,y},$ and $D_{a,y}$ the distributions over $\cX \times \{0,1\} \times \{0,1\}$ given by $D_{\mid A=a}, D_{\mid Y=y}, $ and $D_{\mid A=a, Y=y}$ and $\ellf: \R \times \set{0,1} \to \R_+$ is the user-defined fairness loss with corresponding $\Lf_D(f) := \Ex_{(X, A, Y) \sim D}[\ellf(f(X), Y)]$.
Intuitively, these measure the difference in the average of the fairness loss incurred among the instances with and without the sensitive feature.

Concretely, if $\ellf$ is taken to be $\ellf(s, y) = \1[\sign(s) \neq 1]$ and the 0-1 loss $\ellf(s, y) = \1[\sign(s) \neq y]$ respectively, then 
for $\tau = 0$,
\eqref{eqn:ddp} and \eqref{eqn:deo}
% simplify to
% \begin{align*}
%     %&\textbf{DDP}_{01}: 
%     \Lambda^{\mathrm{DP}}_D( f ) &= \abs{ \mathbb{P}_{D_{0, \cdot}}[ f(X) \geq 0 ] - \mathbb{P}_{D_{1, \cdot}}[ f(X) \geq 0 ] } \\
%     %\leq \tau \\
%     %&\textbf{DEO}_{01}: 
%     \Lambda^{\mathrm{EO}}_D( f ) &= \abs{ \mathbb{P}_{D_{0, 1}}[ f(X) \geq 0 ] - \mathbb{P}_{D_{1, 1}}[ f(X) \geq 0 ] } 
%     %\leq \tau.
% \end{align*}
% For $\tau = 0$,
% these constraints
correspond to the \textit{demographic parity}~\citep{Dwork:2011} and \textit{equality of opportunity}~\citep{Hardt2016} constraints. 
Thus, we denote these two relaxed fairness measures \textit{disparity of demographic parity} (DDP) and \textit{disparity of equality of opportunity} (DEO).
These quantities are also known as the \emph{mean difference score} in~\citet{Calders2010}.% 
\footnote{Keeping $\ellf$ generic allows us to capture a range of group fairness definitions, not just demographic parity and equality of opportunity; e.g., disparate mistreatment~\citep{ZafarWWW} corresponds to using the 0-1 loss and $\Lambda^{\mathrm{DP}}_D$, and equalized odds can be captured by simply adding another constraint for $Y=0$ along with $\Lambda^{\mathrm{EO}}_D$. }

% \footnote{\FINALCHANGE{}{Keeping $\ellf$ generic allows us to capture a range of group fairness definitions, not just demographic parity and equality of opportunity; e.g., disparate mistreatment~\citep{ZafarWWW} corresponds to using the 0-1 loss and $\Lambda^{\mathrm{DP}}_D$, and equalized odds can be captured by simply adding another constraint for $Y=0$ along with $\Lambda^{\mathrm{EO}}_D$. }}
% to be
% \begin{align*}
%     %&\textbf{DDP}: 
%     \Lambda^{\mathrm{DP}}_D( f ) &= |P_{D_{0,\cdot}}[\text{sign}(f(x)=1)]-P_{D_{1,\cdot}}[\text{sign}(f(x)= 1)]| \\
%     %&\textbf{DEO}: 
%     \Lambda^{\mathrm{EO}}_D( f ) &= |P_{D_{0,1}}[\text{sign}(f(x)=1)]-P_{D_{1,1}}[\text{sign}(f(x)= 1)]|.
% \end{align*}

% Sometimes \textit{equalized odds} is required.
% This can be viewed as a special case under the same conditions as the second constraint above and, simultaneously, of the following additional 
% constraint:
% $$\abs{ \Lf_{D_{0, 0}}(f) - \Lf_{D_{1, 0}}(f) } \leq \tau$$
% Although we do not explicitly consider this fairness scenario, all of the results for the generalized equality of 
% opportunity constraint also apply for this third constraint
% %.and having two constraints simultaneously poses no issue.

%\subsection{Balanced error}
%When we regard $Y$ as our target label as usual, we have the following notations:
%\begin{align*}
%    \text{FNR}_y^D(f) &:= \mathbb{P}^-_{D_{\cdot,1}}(f)\\
%    \text{FPR}_y^D(f) &:= \mathbb{P}^+_{D_{\cdot,0}}(f)\\
%    \text{BER}_y^D(f) &:= \frac{\text{FNR}_y^D(f)+\text{FPR}_y^D(f)}{2}
%\end{align*}
%If instead, we regard $A$ as our target label, we have the following notations:
%\begin{align*}
%    \text{FNR}_a^D(f) &:= \mathbb{P}^-_{D_{1,\cdot}}(f)\\
%    \text{FPR}_a^D(f) &:= \mathbb{P}^+_{D_{0,\cdot}}(f)\\
%    \text{BER}_a^D(f) &:= \frac{\text{FNR}_a^D(f)+\text{FPR}_a^D(f)}{2}
%\end{align*}

%

%\begin{table}[h]
%    \centering
%    \begin{tabular}{ll}
%        \toprule
%        \toprule
%         Symbol & Meaning \\
%         \midrule
%         $D_{\cdot, a}$&  \\
%         \bottomrule
%    \end{tabular}
%    \caption{Caption}
%    \label{tab:my_label}
%\end{table}


\begin{table}[t]
\caption {Glossary of commonly used symbols} \label{table:notation}
\centering

\resizebox{0.99\linewidth}{!}{
\begin{tabular}{llll}
\toprule
\toprule
\textbf{Symbol} &  \textbf{Meaning} & \textbf{Symbol} &  \textbf{Meaning} \\ 
\toprule
$X$ &  instance & $D_{\textrm{corr}}$ &  corrupted distribution $D$\\
$A$ &  sensitive feature & $f$ &  score function $f: \cX \to \R$\\
$Y$ &  target feature & $\ellc$ & accuracy loss $\ellc: \R \times \set{0, 1} \to \R_+$ \\
$D$ &  distribution $\mathbb{P}(X,A,Y)$ &  $\Lc_D$ &  expected accuracy loss on $D$\\
$D_{a,\cdot}$ &  distribution $\mathbb{P}(X,A,Y|A=a)$ & $\ellf$ & fairness loss $\ellf: \R \times \set{0, 1} \to \R_+$\\
$D_{\cdot,y}$ &  distribution $\mathbb{P}(X,A,Y|Y=y)$ & $\Lf_D$ & expected fairness loss on $D$ \\
$D_{a,y}$ &  distribution $\mathbb{P}(X,A,Y|A=a,Y=y)$  & $\Lambda_D$ &  fairness constraint  \\ 
\bottomrule
\end{tabular}
}
\end{table}



\subsection{Mutually contaminated learning}
\label{sec:mc-learning}

In the framework of learning from mutually contaminated distributions (MC learning)~\citep{pmlr-v30-Scott13},
instead of observing samples from the ``true'' (or ``clean'') joint distribution $D$,
one observes samples from a corrupted distribution $D_{\mathrm{corr}}$.
The corruption is such that the observed \emph{class-conditional} distributions are mixtures of their true counterparts.
More precisely, let $D_{y}$ denote the conditional distribution for label $y$.
Then, one assumes that
\FINALCHANGE{
\begin{equation}
    \label{equation:mc-model}
    \begin{aligned}
        D_{0, \mathrm{corr}} &= (1-\alpha) \cdot D_{1} + \alpha \cdot  D_{0}\\
        D_{1, \mathrm{corr}} &= \beta \cdot D_{1} + (1-\beta) \cdot  D_{0},
    \end{aligned}
\end{equation}
}{
\begin{equation}
    \label{equation:mc-model}
    \begin{aligned}
        D_{1, \mathrm{corr}} &= (1-\alpha) \cdot D_{1} + \alpha \cdot  D_{0}\\
        D_{0, \mathrm{corr}} &= \beta \cdot D_{1} + (1-\beta) \cdot  D_{0},
    \end{aligned}
\end{equation}
}
where $\alpha, \beta \in (0,1)$ are (typically unknown) noise parameters with $\alpha + \beta < 1$.%
\footnote{\AKMEDIT{The constraint imposes no loss of generality:
when $\alpha+\beta>1$, we can simply flip the two labels and apply our theorem.
When $\alpha+\beta=1$, all information about the sensitive attribute is lost.
This pathological case 
is equivalent to not measuring the sensitive attribute at all.}}
Further, the corrupted base rate $\pi_{\mathrm{corr}} := \mathbb{P}[ Y_{\mathrm{corr}} = 1 ]$ may be arbitrary.
%and in general is distinct from the clean base rate $\pi := \mathbb{P}[ Y = 1 ]$.
The MC learning framework subsumes CCN and PU learning~\citep{pmlr-v30-Scott13,corruption}, \AKMEDIT{which are prominent noise models that have seen sustained study in recent years~\citep{Jain:2017,Kiryo:2017,vanRooyen:2018,Katz:2019,Charoenphakdee:2019}.}
% Thus, it is {a flexible and} appealing noise model.


==> Fairness under corruption NeurIPS 2019 (2)/case_study_privacy.tex <==
%auto-ignore


\begin{figure*}[t]
    \centering
    
    \subfloat[{\tt COMPAS} dataset (privacy case study).]{%
    \includegraphics[width=0.4\textwidth]{img_privacy/{disp_test_compas,0.15,0.15,1.0,DP,Agarwal,3,False}.pdf}
    \includegraphics[width=0.4\textwidth]{img_privacy/{error_test_compas,0.15,0.15,1.0,DP,Agarwal,3,False}.pdf}
    \label{fig:DP_compas}
    }
    
    \subfloat[{\tt law school} dataset (PU learning case study).]{%
    \includegraphics[width=0.4\textwidth]{img_pu_law/{disp_test_law,0.0,0.2,1.0,DP,Agarwal,3,False}.pdf} 
    \includegraphics[width=0.4\textwidth]{img_pu_law/{error_test_law,0.0,0.2,1.0,DP,Agarwal,3,False}.pdf}
    \label{fig:law}
    }
    
    \caption{Relationship between input fairness tolerance $\tau$ versus DP fairness violation (left panels), and versus error (right panels).
    % The %black dotted line 
    % {gray dashed line} represents the ideal fairness violation.
    {Our method ({\sf cor scale}) achieves approximately the ideal fairness violation (indicated by the gray dashed line in the left panels),
    with only a mild degradation in accuracy compared to training on the uncorrupted data (indicated by the {\sf nocor} method).
    Baselines that perform no noise-correction ({\sf cor})
    and explicitly denoise the data ({\sf denoise})
    offer suboptimal tradeoffs by comparison;
    for example, the former achieves slightly lower error rates, but does so at the expense of greater fairness violation.}}
\end{figure*}

In this case study, we look at {\tt COMPAS}, a dataset from Propublica~\citep{COMPAS} that is widely used in the study of fair algorithms.
Given various features about convicted individuals, the task is to predict recidivism and the sensitive attribute is race.
The data comprises 7918 examples and 10 features.
In our experiment, we assume that to preserve differential privacy, 
CCN noise with 
%$\rho^+=\rho^- \in \set{0.15, 0.3}$ 
{$\rho^+=\rho^- = {0.15}$}
is added to the sensitive attribute. 
As per {Lemma} \ref{thm: randomized response for differential privacy}, this guarantees $(\epsilon, \delta=0)$ differential privacy with 
%$\epsilon \in \set{1.73, 0.85}$ respectively. 
{$\epsilon = {1.73}$.}
We assume that the noise level $\rho$ is released with the dataset (and is thus known). 
We performed fair classification on this noisy data using our method and compare the results to the three benchmarks described above.

Figure \ref{fig:DP_compas} shows the average result over three runs each with a random 80-20 training-testing split.
(Note that fairness violations and errors are calculated with respect to the true uncorrupted features.)
{We draw two key insights from this graph:}
\begin{enumerate}[label=(\roman*),itemsep=-2pt,topsep=0pt,leftmargin=24pt]
    \item {in terms of fairness violation,
    our method ({\sf cor scale}) approximately achieves the desired fairness tolerance (shown by the {gray dashed} line).}
    This is both expected and ideal, and it matches what happens when there is no noise ({\sf nocor}).
    By contrast, the na\"{i}ve method {\sf cor} strongly violates the fairness constraint.

    \item {in terms of accuracy, 
    our method only suffers mildly
    compared with the ideal noiseless method ({\sf nocor});
some degradation} is expected as noise will lead to some loss of information.
By contrast, {\sf denoise} sacrifices much more {predictive} accuracy than our method.

    % \item our method ({\sf cor scale}) achieves the best accuracy while respecting the desired fairness tolerance.
    % This is evidenced by
    % the red line being below the gray dashed line (Figure~\ref{fig:DP_compas}, left panel).

%     \item \AKMEDIT{the other baselines fare worse than our method:}
% indeed, as expected, the na\"{i}ve method {\sf cor} violates the fairness constraint.
% While {\sf denoise} achieves the desired fairness level, it has large fluctuations and sacrifices much more {predictive} accuracy than our method.
% \AKMEDIT{Finally, while the {\sf cor} method achieves slightly lower error rates, it does so at the expense of greater fairness violation.}
\end{enumerate}
In light of both the above, our method is seen to achieve the best overall tradeoff between fairness and accuracy.
{Experimental results with EO constraints,
and other commonly studied datasets in the fairness literature ({\tt adult}, {\tt german}), 
show similar trends as}
%We also tried using the EO constraint as well as other datasets. The results obtained showed the same trends that are observable 
in Figure \ref{fig:DP_compas}, and are included in Appendix \ref{appendix:privacy} for completeness.

% The sensitive attribute race is hard to be learned when it is regarded as the target label, even when no noise is present, \cite{northcutt2017rankpruning} with SVM with rbf kernel as the base classifier can only get $65\%$ accuracy when no noise is present, which is even worse than using the corrupted labels. It can also get $65$ when $\rho_a^+=\rho_a^-=0.2$. When $\rho_a^+=\rho_a^-=0.4$, its accuracy decreases to $60\%$.







==> Fairness under corruption NeurIPS 2019 (2)/case_study_pu.tex <==
%auto-ignore

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.4\textwidth]{img_pu_law/{disp_test_law,0.0,0.2,1.0,DP,Agarwal,3,False}.pdf} 
%     \includegraphics[width=0.4\textwidth]{img_pu_law/{error_test_law,0.0,0.2,1.0,DP,Agarwal,3,False}.pdf}

%     \caption{Relationship between input $\tau$ and fairness violation/error on the {\tt law school} dataset using DP constraint (testing curves).
%     % The %black dotted 
%     % {gray dashed line} represents the ideal fairness violation.
%     % Note that in some of the graphs, the red line and the orange line perfectly overlap with each other.
%     \AKMEDIT{Our method {\sf cor scale} closely achieves approximately the ideal violation (indicated by the gray dashed line in the left panel),
%     with only a mild degradation in accuracy compared to training on the uncorrupted data (indicated by the {\sf nocor} method in the right panel).}    
%     }
%     \label{fig:law}
% \end{figure*}

% AKM: only use #1 and #3
% emphasise directly that red line is closer to yellow
% green is super-fair and erroneous
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{{img_pu_law_noise_est/disp_test_law,0.0,0.2,1,DP,Agarwal,3,False,test_rho_est_err}.pdf}
    \includegraphics[width=0.4\textwidth]{{img_pu_law_noise_est/error_test_law,0.0,0.2,1,DP,Agarwal,3,False,test_rho_est_err}.pdf}
    \caption{Relationship between the estimated noise level $\hat{\rho}^-$ and fairness violation/error on the {\tt law school} dataset using DP constraint (testing curves), with $\hat{\rho}^+ = 0$ and $\tau=0.2$. Our method ({\sf cor scale}) is not overly sensitive to imperfect estimates of the noise rate, evidenced by its fairness violation and accuracy closely tracking that of training on the uncorrupted data ({\sf nocor})
    as $\hat{\rho}^-$ is varied. That is, red curve in the left plot closely tracks the yellow reference curve.
    By contrast, the baseline that explicitly denoises the data ({\sf denoise}) deviates strongly from {\sf nocor},
    and is sensitive to small changes in $\hat{\rho}^-$.
    This illustrates that our method performs well even when noise rates must be estimated.}
    \label{fig:law_est_err}
\end{figure*}


%Table \ref{Tab:noise} shows the influence of this noise on the size of both sensitive groups for the training set.
%
%\begin{table}[ht]
%\caption{Impact of noise on two groups}
%\centering
%\begin{tabular}{ | l | l | l |}
%    \hline
%    situations & $A=0$ & $A=1$ \\ \hline
%    w/o noise & 978 & 2012 \\ \hline
%    w/ noise $\rho_a^-=0.2$ & 765 & 2225 \\ \hline
%    w/ noise $\rho_a^-=0.4$ & 567 & 2423 \\ \hline
%\end{tabular}
%\label{Tab:noise}
%\end{table}

In this case study, we consider the dataset {\tt law school}, which is a subset of the original dataset from LSAC~\citep{Wightman}. In this dataset, one is provided with information about various individuals (grades, part time/full time status, age, etc.) and must determine whether or not the individual passed the bar exam.
The sensitive feature is race; we only consider black and white.
After prepossessing the data by removing instances that had missing values and those belonging to other ethnicity groups (neither black nor white) we were left with 3738 examples each with 11 features. 

While the data ostensibly provides the true values of the sensitive attribute, one may imagine having access to only PU information.
Indeed, when the data is collected one could imagine that individuals from the minority group would have a much greater incentive to %lie about
{conceal} their group membership due to fear of discrimination.
% Note that there would be no similar incentive if belonging to the majority group.
Thus, any individual identified as belonging to the majority group could be assumed to have been correctly identified (and would be part of the positive instances).
On the other hand, no definitive conclusions could be drawn about individuals identified as belonging to the minority group (these would therefore be part of the unlabelled instances). 

To model a PU learning scenario, we added CCN noise to the dataset with $\rho^+ = 0$ and 
%$\rho^- \in \set{0.2, 0.4}$. 
{$\rho^- = {0.2}$.}
% Again, we perform fair classification on this noisy dataset with DP as the constraint. 
% We use our method as well as the three benchmarks described above.
We initially assume that the noise rate is known. %(some kind of perfect estimator is available).
Figure \ref{fig:law} shows the average result over three runs under this setting each with a random 80-20 training-testing split. 
{We draw the same conclusion as before:
our method
achieves the highest accuracy while
respecting the specified fairness constraint.
% nearly achieves the ideal fairness violation, 
% while only slightly degrading in terms of accuracy.
% Further, the other baselines yield worse tradeoffs than our method.
}
% As before, it can be seen that the na\"{i}ve method {\sf cor} violates the fairness constraint while our method {\sf cor scale} reaches a degree of fairness violation which is very close to the level reached by the fair classifier when there is no noise ({\sf nocor}).
% Although the method {\sf denoise} seems to also achieve the desired fairness level, it does so by sacrificing much more accuracy than our method.

Unlike in the privacy case, the noise rate in the PU learning scenario is usually unknown in practice,
and must be estimated.
%Many methods exist that can be used to estimate the noise rate.
{Such estimates will inevitably be approximate.}
We thus evaluate the impact of the error of the noise rate estimate on all methods.
%in terms of accuracy and fairness violation.
{In Figure~\ref{fig:law_est_err}, we consider a PU scenario where 
%$\rho^+=0$ is known, but 
we only have access to an estimate $\hat{\rho}^-$ of the negative noise rate,
whose true value is $\rho^- = 0.2$.}
Figure \ref{fig:law_est_err} shows the impact of different values of $\hat{\rho}^-$ on the fairness violation and error.
We see that that as long as this estimate is reasonably accurate, 
our method performs the best in terms of being closest to the case of running the fair algorithm on uncorrupted data.

%\aditya{Minimizing, US english.}
In sum,
these results are consistent with our derivation and show that our method {\sf cor scale} can achieve the desired degree of fairness while minimising loss of accuracy.
Appendix \ref{appendix:pu} includes results for different settings of $\tau$, noise level, and on other datasets showing similar trends.


==> Fairness under corruption NeurIPS 2019 (2)/conclusion.tex <==
%auto-ignore
In this paper, we showed both theoretically and empirically that even under the very general MC learning noise model~\citep{Scott13} on the sensitive feature, fairness can still be preserved by scaling the input unfairness tolerance parameter $\tau$.
% Our method can be applied before any downstream classifiers (that takes in a parameter $\tau$ that is proportional to mean-difference score of some fairness measures).
% We also provide applications in PU-learning and privacy preservation.
In future work, it would be interesting to consider the case of categorical sensitive attributes (as applicable, e.g., for race),
and the more challenging case of instance-dependent noise~\citep{Awasthi:2015}.
% Further, considering the case of handling noisy $A$ when the latter is used as input to the classifier would also be of interest.
\AKMEDIT{We remark also that in independent work,~\citet{Awasthi:2019} studied the effect of sensitive attribute noise on the post-processing method of~\citet{Hardt2016}.
In particular, they 
identified conditions when such post-processing can still yield an approximately fair classifier.
Our approach has an advantage of being applicable to a generic in-processing fair classifier;
however, their approach also handles the case where the sensitive feature is used as an input to the classifier.
Exploration of the synthesis of the two approaches is another promising direction for future work.
}


==> Fairness under corruption NeurIPS 2019 (2)/experiment_sanity_check.tex <==
%auto-ignore
\iffalse




% \subsubsection{Assuming we know noise rates}
% \label{ssec:num1:known_nr}

Following a large number of previous studies,
we use four datasets for our experiments:
\begin{itemize}[itemsep=0pt,topsep=0pt]
    \item {\tt adult}, a dataset from the UCI repository~\citep{UCI}.
    The task is to predict if one's annual income is more than 50k and the sensitive attribute is gender or race. 
    The data comprises 48842 examples and 14 features.

    \item {\tt german}, another dataset from the UCI repository~\citep{UCI}. The task is to predict if one has good credit and the sensitive attribute is if a person is foreign.
    The data comprises 1000 examples and 20 features.
    
    \item {\tt Law School}, a dataset from LSAC~\citep{Wightman}.
    The task is to predict the passage of the bar exam and the sensitive attribute is race. 
    The data comprises 16638 examples and 11 features.
    
    \item {\tt COMPAS}, a dataset from Propublica~\citep{COMPAS}.
    The task is to predict recidivism and the sensitive attribute is race.
    The data comprises 7918 examples and 10 features.
    

\end{itemize}

We now present experiments in several progressively challenging settings:
where there is noise in $A$,
and where the noise aims to preserve privacy.


%
\subsection{Noise in the sensitive attribute}

For simplicity, we add noise according to CCN model, i.e. we randomly flip the sensitive attribute of samples with $A = 1$ with probability $\rho^+$ and randomly flip the sensitive attribute of samples with $A = 0$ with probability $\rho^-$.
For further simplicity, we let $\rho:=\rho^+=\rho^-$.

We present results first assuming prior knowledge of the noise rates,
and then where the noise rates are estimated from data.


%
% \subsubsection{Assuming we know noise rates}
% \label{ssec:num1:known_nr}

We assume that we know the values of $\rho$. In this case, we can estimate $\alpha$ and $\beta$ using relationship specified in 3.3.2.

As a baseline (termed {\sf denoise}) and then apply \cite{reduction}. We apply the {\sf RankPrune} method in \cite{northcutt2017rankpruning} to denoise $A$. {\sf denoise} is a two-steps method, it first estimate noise rates and then estimate A based on the estimated noise rates. For the purpose of fair comparison, we pass the known noise rates to {\sf denoise} and only use its second step in this section.

Our method (termed {\sf cor\_scale}) scales the input parameter $\tau$ and then ~\citet{reduction} to perform fair classification.

We run experiments at noise level $\rho=0.2$ on both {\tt adult} and {\tt COMPAS}.

We compare the relationship between the input $\epsilon$ and training/testing error/fairness violation under both DP and EO of four situations.

\begin{itemize}
    \item Apply \cite{reduction} on no-corrupted data(termed {\sf nocor}).
    \item Apply \cite{reduction} on corrupted data(termed {\sf cor}).
    \item {\sf denoise}
    \item {\sf cor scale}
\end{itemize}

Each plot is the average of three runs. At each run, we make a random $80$--$20$ train-test split.

The $x$-axis is the given input $\tau$ that controls the strictness of fairness constraint and $y$-axis is DEO or DDP as defined in \ref{section:fairnessdef}.

It can be seen from Figures~\ref{fig:DP_compas_known} and \ref{fig:EO_compas_known} that the fairness violation and error rates of {\sf cor\_scale} are much closer to {\sf no\_cor} when compared with both {\sf cor} and {\sf denoise} under both DP and EO.

This result is consistent with our derivation and implies that our scaling indeed helps to achieve the originally wanted degree of fairness before corruption.
Besides, without surprise, due to down-scaling the $\epsilon$, the corruption with scaling causes slightly higher error than the {\sf no\_cor} for both datasets on both training set and testing set.

See Appendix \ref{appendix:knowing-nr-training} for the corresponding results on the training set.

See Appendix \ref{appendix:noise-level} for the same experiment performed at different noise levels.
\fi




\iffalse
\subsubsection{Assuming we do not know noise rates}

We next turn to the more realistic (but challenging) setting where the noise rates are unknown.
Here, as a baseline (termed {\sf denoise}), we apply the {\sf RankPrune} method in \cite{northcutt2017rankpruning} to denoise $A$, and then apply \cite{reduction}.
Our method (termed {\sf scale\_est}) follows Algorithm~\ref{alg:reduction},
employing {\sf RankPrune} to estimate $\rho^+$ and $\rho^-$ (and thus $\hat{\alpha}_a$ and $\hat{\beta}_a$),
and then ~\citet{reduction} to perform fair classification.

We use the same setup as before (except choosing $\rho=0.3$ to see clearer pattern). We compare the training/testing fairness violation/error rate of the two methods at different input $\epsilon$. For the purpose of comparison, we also include the three curves specified in the previous section.

It can be seen from Figure~\ref{fig:DP_compas_five} that our method produces better preservation of fairness requirement compared with the baseline method.

\begin{center}
    \includegraphics[width=0.4\textwidth]{imgs2/DP_Agarwal_compas_03_3_ref_five}
    \captionof{figure}{(DP) Relationship between input epsilon and fairness violation/error on the UCI {\tt adult} dataset.}
    \label{fig:DP_compas_five}
\end{center}
\fi

==> Fairness under corruption NeurIPS 2019 (2)/intro.tex <==
%auto-ignore
Classification is concerned with maximally discriminating between a number of pre-defined groups.
%(e.g., determining if an individual is likely to repay a loan, or not).
\emph{Fairness-aware} classification concerns the analysis and design of classifiers that
do not discriminate with respect to some sensitive feature (e.g., race, gender, age, income).
Recently, much progress has been made
on devising {appropriate} measures of fairness~\citep{Calders,Dwork:2011,Feldman,Hardt2016,ZafarWWW,Zafar:2017b,Kusner,Kim,Speicher:2018,Heidari:2019},
and
means of achieving them~\citep{ZemelICML,ZafarWWW,Calmon:2017,Dwork:2018,reduction,Donini:2018,Cotter:2018,Williamson:2019,Mohri:2019}.

Typically, fairness is achieved by adding constraints which depend on the sensitive feature, and then correcting one's learning procedure to achieve these fairness constraints.
For example, suppose the data comprises of pairs of individuals and their loan repay status,
and the sensitive feature is gender.
Then, we may add a constraint that we should predict equal loan repayment for both men and women (see \S\ref{section:fairnessdef} for a more precise statement).
However, this and similar approaches assume that we are able to correctly measure or obtain the sensitive feature. 
In many real-world cases, one may only observe noisy versions of the sensitive feature.
For example, survey respondents may choose to conceal or obfuscate their group identity out of %privacy concerns.
{concerns of potential mistreatment or outright discrimination}. 

One is then brought to ask whether fair classification in the presence of such \emph{noisy} sensitive features is still possible.
Indeed, if the noise is high enough and all original information about the sensitive features is lost, then it is as if the sensitive feature was not provided.
Standard learners can then be 
%\aditya{I don't know if ``necessarily'' is true.}
%\EDIT{necessarily} 
unfair on such data~\citep{Dwork:2011, pedreshi2008discrimination}.
Recently,~\citet{hashimoto2018fairness} showed that progress is  possible, albeit for specific fairness measures.
%(and potentially impossible).
The question of what can be done under a smaller amount of noise is thus both interesting and non-trivial.

In this paper, we consider two {practical} scenarios where we may only observe noisy sensitive features:
\begin{enumerate}[itemsep=0pt,topsep=0pt,leftmargin=16pt,label={(\arabic*)}]
    \item suppose we are releasing data involving human participants.
    %Even if noise-free sensitive features are available,
    %for legal or ethical reasons,
    %we may wish to \emph{add} noise so as to obfuscate sensitive attributes,
    %and thus protect the participants' privacy.
    % \EDIT{Even if noise-free sensitive features are available,
    % we may wish to \emph{add} noise so as to obfuscate sensitive attributes, for legal or ethical reasons
    % to protect participant data from potential misuse.}
    Even if noise-free sensitive features are available,
    we may wish to \emph{add} noise so as to obfuscate sensitive attributes,
    and thus protect participant data from potential misuse.
    % in some cases, while the noise-free sensitive feature might be available, it may be desirable to add noise to it before being able to publish the data.
    % Indeed, one might legally or ethically have to obfuscate sensitive attributes so as to protect the privacy of a study's participants.
    Thus, being able to learn fair classifiers under sensitive feature noise is a way to achieve both privacy \emph{and} fairness.
    
    \item suppose we wish to analyse data where 
    the presence of the sensitive feature is only known for a subset of individuals,
    while for others the feature value is unknown.
    For example,
    % consider a historical dataset where the presence of the sensitive feature (e.g., disability) was occasionally recorded.
    % Alternatively,
    patients filling out a form may feel comfortable disclosing that they do not have a pre-existing medical condition; however, some who do have this condition may %not provide truthful responses.   
    {wish to refrain from responding}.
    This can be seen as a variant of the \emph{positive and unlabelled} (PU) setting~\citep{Denis:1998a},
    where the sensitive feature is present (positive) for some individuals,
    but absent (unlabelled) for others.
    % The sensitive feature can be considered  (positive points) but where most entries could have been either positive or negative (thus unlabelled points).
    % we consider cases where 
    % That is, rather than being able to tell whether the sensitive feature is positive or negative, we are simply given positive and unlabeled entries.
\end{enumerate}

%By considering a general measure of fairness and model of noise, 
By considering {popular measures of fairness and a general model of noise},
we show that fair classification is possible under 
%many (including the above) settings.
many settings, including the above.
Our precise contributions are:
\begin{enumerate}[itemsep=0pt,topsep=0pt,leftmargin=24pt,label=(\textbf{C\arabic*})]
    \item we show that if the sensitive features are subject to noise as per the \emph{mutually contaminated learning model}~\citep{Scott13},
and one measures fairness using the \emph{mean-difference score}~\citep{Calders2010},
then a simple identity (Theorem~\ref{thm: sensitive noise reduction}) yields that we only need to change the desired fairness-tolerance.
The requisite tolerance can be estimated by leveraging existing noise-rate estimators
from the label noise literature,
% \AKMEDIT{from the label noise literature},
yielding a reduction (Algorithm~\ref{alg:reduction}) to regular noiseless fair classification.

    \iffalse \item We additionally show that the framework can handle noise in both the sensitive \emph{and} target feature.\fi

    \item we show that our procedure is empirically effective on both case-studies mentioned above.
    %in which the sensitive feature is purposefully obfuscated for privacy reasons, or only available in the PU setting.
\end{enumerate}

In what follows,
we review the existing literature on learning fair and noise-tolerant classifiers in~\S\ref{sec:related},
and introduce the %(to our knowledge novel)
novel
problem formulation of noise-tolerant fair learning %in~\S\ref{sec:problem-formulation}.
in~\S\ref{sec:background}.
We then detail how to address this problem in~\S\ref{section:sensnoise},
and empirically confirm the efficacy of our approach in~\S\ref{sec:experiments}.


==> Fairness under corruption NeurIPS 2019 (2)/noise_on_a.tex <==
%auto-ignore
The standard fairness-aware learning problem assumes we have access to the true sensitive attribute,
so that we can both measure and control our classifier's unfairness as measured by, e.g., Equation~\ref{eqn:ddp}.
Now suppose that rather than being given the sensitive attribute, we get a noisy version of it. 
We will show that the fairness constraint on the clean distribution is \emph{equivalent} to a \emph{scaled} constraint on the 
noisy distribution.
% That is,
% we show that fairness constraints are naturally robust to noise in the sensitive attribute.
This gives a simple reduction from fair machine learning in the presence of noise to
the regular fair machine learning, which can be done in a variety of ways as discussed in~\S\ref{sec:bg-fairness}.

%
\subsection{Sensitive attribute noise model}
\label{section:sensnoisesetup}

\iffalse
To design a suitable noise model, let us consider two plausible settings wherein the observed sensitive feature $A$ may not be reflective of the ground-truth:
\begin{itemize}[itemsep=0pt,topsep=0pt]
    \item the \emph{obfuscation} setting, wherein some individuals decide to purposely obfuscate their sensitive feature,
    perhaps for fear of being the subject of algorithmic discrimination.
    For example, applicants to a job may be way of disclosing their race.

    \item the \emph{opt-out} setting, wherein some individuals decide to provide a sensitive feature, but others decide to abstain from providing this information, perhaps over concerns of privacy.
    For example, patients filling out a medical form may feel comfortable disclosing that they do not have a pre-existing medical condition;
    however, those who do have this condition may not provide truthful responses.
\end{itemize}
The former can be modelled as a form of class-conditional noise (CCN) on $A$,
where each individual makes an independent decision whether or not to provide their true value of $A$ or not.%
\footnote{This assumption of instance-independent noise is unlikely to hold exactly in practice. Nonetheless, we believe it to be a useful first step in studying the effects of noise on fairness-aware learning methods.}
The latter can be modelled as a form of positive unlabelled (PU) learning,
where only a subset of individuals with a sensitive feature decide to reliably provide that information.

To capture both types of noise in the sensitive attribute,
we adopt the framework of learning from mutually contaminated distributions (MC learning)~\cite{pmlr-v30-Scott13},
as introduced in \S\ref{sec:mc-learning}.
Our choice is motivated by the fact that MC learning captures both PU and CCN learning as special cases;
hence, our results imply results for both of these interesting special cases. 
\fi

As previously discussed, we use MC learning as our noise model,
as this captures both CCN and PU learning as special cases;
hence, we automatically obtain results for both these interesting settings.

Our specific formulation of MC learning noise on the sensitive feature is as follows.
Recall from \S\ref{section:fairnessdef} that $D$ is a distribution over $\mathscr{X} \times \set{0,1} \times \set{0,1}$.
Following (\ref{equation:mc-model}),
for unknown noise parameters
$\alpha,\beta \in (0,1)$ with $\alpha + \beta < 1$,
we assume that the corrupted class-conditional distributions are:
\begin{equation}\label{equation:mcnoise1}
    \begin{aligned}
        &D_{1,\cdot,\mathrm{corr}} = (1-\alpha) \cdot D_{1,\cdot} + \alpha \cdot  D_{0,\cdot}\\
        &D_{0,\cdot,\mathrm{corr}} = \beta \cdot D_{1,\cdot} + (1-\beta) \cdot  D_{0,\cdot},
    \end{aligned}
\end{equation}
and that the corrupted base rate is $\pi_{a,\mathrm{corr}}$ (we write the original base rate, $\mathbb{P}_{(X, A, Y) \sim D}[A=1]$ as $\pi_a$).
%In words,
{That is,} the distribution over (instance, label) pairs for the group with $A = 1$, i.e. $\mathbb{P}( X, Y \mid A = 1 )$,
is assumed to be mixed with the distribution for the group with $A = 0$, and vice-versa.

Now, when interested in the EO constraint, it can be simpler to assume that the noise instead satisfies
\begin{equation}\label{equation:mcnoise2}
    \begin{aligned}
        &D_{1,1,\mathrm{corr}} = (1-\alpha') \cdot D_{1,1} + \alpha' \cdot D_{0,1}\\
        &D_{0,1,\mathrm{corr}} = \beta' \cdot D_{1,1} + (1-\beta') \cdot D_{0,1},
    \end{aligned}
\end{equation}
for noise parameters $\alpha', \beta' \in (0, 1)$.
As shown by the following, this is not a different assumption.
%but simply a direct implication of \eqref{equation:mcnoise1}. 

\begin{lemma}\label{lemma:mcrelation}
    Suppose there is noise in the sensitive attribute only, as given in Equation \eqref{equation:mcnoise1}.
    Then,
    there exists constants $\alpha', \beta'$ such that
    Equation \eqref{equation:mcnoise2} holds.
    % \begin{align*}
    % \alpha' &= \frac{\alpha\mathbb{P}[Y=1 \mid A = 0] }{(1-\alpha)\mathbb{P}[Y=1 \mid A = 1] + \alpha \mathbb{P}[Y=1 \mid A=0]} \\
    % \beta' &= \frac{\beta\mathbb{P}[Y=1 \mid A = 1] }{(1-\beta)\mathbb{P}[Y=1 \mid A = 0] + \beta \mathbb{P}[Y=1 \mid A=1]}
    % \end{align*}
\end{lemma}

% In the proof of Lemma~\ref{lemma:mcrelation}, we see
% that $\alpha=\alpha'$ when $Y \independent A$, i.e., $\mathbb{P}[Y=1|A=0]=\mathbb{P}[Y=1|A=1]$.
% However, in practice this will rarely be the case as it implies there is no intrinsic unfairness.
% Furthermore,
Although the lemma %shows that \eqref{equation:mcnoise1} implies \eqref{equation:mcnoise2} and
gives a way to calculate $\alpha', \beta'$ from $\alpha, \beta$, in practice it may be useful to consider \eqref{equation:mcnoise2} independently.
Indeed, when one is interested in the EO constraints we will show below that only knowledge of $\alpha', \beta'$ is required.
%Rather than estimating all of $\alpha, \beta, \mathbb{P}[Y=1 | A=1],$ and $\mathbb{P}[Y=1 | A=0]$
It is often much easier to estimate $\alpha', \beta'$ directly
(which can be done in the same way as estimating $\alpha, \beta$ simply by considering $D_{\cdot, 1, \mathrm{corr}}$ rather than $D_{\mathrm{corr}}$).


%
\subsection{Fairness constraints under MC learning}

We now show that the previously introduced fairness constraints for demographic parity and equality of opportunity are automatically robust to MC learning noise in $A$.

\begin{theorem}\label{thm: sensitive noise reduction}
    Assume that we have noise as per Equation \eqref{equation:mcnoise1}.
    Then, for any $\tau > 0$ and $f \colon X \to \mathbb{R}$,
    \begin{align*}
    %  &\abs{\Lf_{D_{0,\cdot}}(f)-\Lf_{D_{1,\cdot}}(f)} \leq \tau \iff \\ &\abs{\Lf_{D_{0,\cdot, \text{corr}}}(f)-\Lf_{D_{1,\cdot, \text{corr}}}(f)} \leq \tau(1-\alpha - \beta).
     \Lambda^{\mathrm{DP}}_{D}( f ) \leq \tau &\iff \Lambda^{\mathrm{DP}}_{D_{\mathrm{corr}}}(f) \leq \tau \cdot (1-\alpha - \beta) \\
    %\end{align*}
    %Additionally, for the EO-like constraints,
    %\begin{align*}
        % &\abs{\Lf_{D_{0,1}}(f)-\Lf_{D_{1,1}}(f)} \leq \tau \iff \\
        % &\abs{\Lf_{D_{0,1, \text{corr}}}(f)-\Lf_{D_{1,1, \text{corr}}}(f)} \leq \tau(1-\alpha' - \beta'),        
         \Lambda^{\mathrm{EO}}_{D_{\cdot, 1}}( f ) \leq \tau &\iff \Lambda^{\mathrm{EO}}_{D_{\mathrm{corr}, \cdot, 1}}(f) \leq \tau \cdot (1-\alpha' - \beta'),
    \end{align*}
    where $\alpha'$ and $\beta'$ are as per Equation~\eqref{equation:mcnoise2} and Lemma~\ref{lemma:mcrelation}.
\end{theorem}

The above can be seen as a consequence of the immunity of the \emph{balanced error}~\citep{Chan:1998,Brodersen:2010,consistency} to corruption under the MC model.
Specifically, consider a distribution $D$ over an input space $\mathscr{Z}$ and label space $\mathscr{W} = \set{0, 1}$.
Define
$$ B_{D} := \mathbb{E}_{Z \mid W = 0}[ h_0( Z ) ] + \mathbb{E}_{Z \mid W = 1}[ h_1( Z ) ] $$
for functions $h_0, h_1 \colon \mathscr{Z} \to \R$.
% This is a generalised form of balanced error, being the average of false positive and negative rates of a classifier.
Then, if for every $z \in \mathbb{R}$
$h_0( z ) + h_1( z ) = 0$, %is a constant,
we have~\citep[Theorem 4.16]{vanRooyen:2015}, \citep{Blum:1998,Zhang:2008,corruption}
\begin{equation}
    \label{eqn:ber-identity}
     B_{D_{\mathrm{corr}}} = (1 - \alpha - \beta) \cdot B_{D},%+ \frac{\alpha + \beta}{2},    
\end{equation}
where $D_{\mathrm{corr}}$ refers to a corrupted version of $D$ under MC learning with noise parameters $\alpha, \beta$.
%In words, 
{That is,} the effect of MC noise on $B_D$ is simply to perform a scaling.
Observe that
$B_D = \Lf_D( f )$
if
we set
%$\mathscr{Z} = \mathscr{X} \times \set{0, 1}$,
$Z$ to $X \times Y$,
$W$ to the sensitive feature $A$,
and
% \begin{align*}
%     h_0( (x, y) ) &= +\ellf( y, f( x ) ) \\
%     h_1( (x, y) ) &= -\ellf( y, f( x ) ).
% \end{align*}
$h_0( (x, y) ) = +\ellf( y, f( x ) )$,
$h_1( (x, y) ) = -\ellf( y, f( x ) )$.
Thus, (\ref{eqn:ber-identity}) implies $\Lf_D( f ) = (1 - \alpha - \beta) \cdot \Lf_{D_{\mathrm{corr}}}( f )$,
and thus Theorem~\ref{thm: sensitive noise reduction}.



%
\subsection{Algorithmic implications}

Theorem~\ref{thm: sensitive noise reduction} has an important algorithmic implication.
Suppose we pick a fairness constraint $\Lambda_D$ and seek to solve
Equation~\ref{eqn:fairness-objective} for a given tolerance $\tau \geq 0$.
Then,
given samples from $D_{\mathrm{corr}}$, it suffices to simply change the tolerance to $\tau' = \tau \cdot (1 - \alpha - \beta)$.

Unsurprisingly, $\tau'$ depends on the noise parameters $\alpha, \beta$.
In practice, these will be unknown;
however, there have been several algorithms proposed to estimate these from noisy data alone~\citep{pmlr-v30-Scott13,corruption,Liu2016ClassificationWN,Ramaswamy:2016,northcutt2017rankpruning}.
Thus, we may use these to construct estimates of $\alpha, \beta$, and plug these in to construct an estimate of $\tau'$.

In sum, we may tackle fair classification in the presence of noisy $A$ by suitably combining \emph{any} existing fair classification method (that takes in a parameter $\tau$ that is proportional to mean-difference score of some fairness measures), and \emph{any} existing noise estimation procedure.
This is summarised in Algorithm~\ref{alg:reduction}.
Here, {\sf FairAlg} is any existing fairness-aware classification method that solves Equation~\ref{eqn:fairness-objective}, and {\sf NoiseEst} is any noise estimation method that estimates $\alpha, \beta$.

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
	\caption{Reduction-based algorithm for fair classification given noisy $A$.}
	\label{alg:reduction}
	\begin{algorithmic}[1]
	    \REQUIRE Training set $S = \{ (x_i, y_i, a_i) \}_{i=1}^n$,
	    scorer class $\cF$,
	    fairness tolerance $\tau \geq 0$,
	    fairness constraint $\Lambda( \cdot )$,
	    fair classification algorithm {\sf FairAlg},
	    noise estimation algorithm {\sf NoiseEst}
	    \ENSURE  Fair classifier $f^* \in \cF$
	    \STATE   $\hat{\alpha}, \hat{\beta} \leftarrow {\sf NoiseEst}( S )$
	    \STATE   $\tau' \leftarrow ( 1 - \hat{\alpha} - \hat{\beta} ) \cdot \tau$
	    \STATE  \textbf{return} ${\sf FairAlg}( S, \cF, \Lambda, \tau' )$
	\end{algorithmic}
\end{algorithm}


%
%\subsection{Practical implications}
%
%When data gets released it is often necessary to protect the identities of those that the data pertains to. 
%%This is especially true for medical data or data from the social sciences.
%While this concern pervades all areas of machine learning, it is particularly important in the context of fair learning since those same datasets are often the ones where fairness is a major concern.
%%While anonymization is sometimes enough, there are cases where stronger steps have to be taken in order to protect the participant's privacy.
%
%Surprisingly, our result immediately gives an extraordinarily simple and relatively effective method to protect privacy while still allowing for fair classification. Indeed, consider simply adding CCN noise to the sensitive attribute (and perhaps other features) of the of dataset instances. While this does not protect against multiple stronger privacy attacks, it does give some assurance that an instance's true features (and thus hopefully its identity) cannot be recovered with 100\% certainty. Meanwhile our result implies that fair classification would still be possible. Furthermore, it gives a way to achieve fair classification by simply scaling $\tau$ as per Theorem \ref{thm: sensitive noise reduction} before calling any of a large group of downstream fair classifiers with several options as to which group fairness constraint to use.
%
%There are many real world cases in which a PU setting for the sensitive attribute is very realistic. Indeed, one may be able to clearly identify some instances of the minority group while being unable to tell whether the rest of the instances were in the majority or minority groups.

%

\FINALCHANGE{}{\subsection{Noise rate and sample complexity}

So far, we have shown that at a distribution level, fairness with respect to the noisy sensitive attribute is equivalent to fairness with respect to the real sensitive attribute. 
However, from a sample complexity perspective, a higher noise rate will require a larger number of samples for the empirical fairness to generalize well, i.e., guarantee fairness at a distribution level. 
A concurrent work by~\citet{fairlearning_withprivatedata} derives precise sample complexity bounds and makes this relationship explicit.
}







\subsection{Connection to \FINALCHANGE{differential privacy}{privacy and fairness}}

While Algorithm \ref{alg:reduction} gives a way of achieving fair classification on an already noisy dataset such as the {use case} described in example (2) of \S\ref{sec:intro}, it can also be used to simultaneously achieve fairness and privacy.
As described in example (1) of \S\ref{sec:intro}, the very nature of the sensitive attribute makes it likely that even if noiseless sensitive attributes are available, one might want to add noise to guarantee some form of privacy.
Note that {simply} removing the feature does not suffice, because it would make difficult the task of
% \AKMEDIT{make difficult the task of}
developing fairness-aware classifiers for the dataset
% \AKMEDIT{~\citep{Gupta:2018}}.
~\citep{Gupta:2018}.
Formally, we can give the following privacy guarantee by adding CCN noise to the sensitive attribute. 

\begin{lemma}\label{thm: randomized response for differential privacy}
    To achieve $(\epsilon, \delta=0)$ differential privacy
    on the sensitive attribute we can add CCN noise with $\rho^+ = \rho^- = \rho \geq \frac{1}{\exp{(\epsilon)}+1}$ to the sensitive attribute.
\end{lemma}

Thus, if a desired level of differential privacy is required before releasing a dataset, one could simply add the required amount of CCN noise to the sensitive attributes, publish this modified dataset as well as the noise level, and researchers could use Algorithm \ref{alg:reduction} (without even needing to estimate the noise rate) to do fair classification as usual. 

\FINALCHANGE{Recently,~\citet{Kearns18} explored preserving differential privacy~\citep{Dwork06} while %at the same time of preserving 
{maintaining} fairness constraints.}{There is previous work that tries to preserve privacy of individuals' sensitive attributes while learning a fair classifier.
\cite{pmlr-v80-kilbertus18a} employs the cryptographic tool of secure multiparty computation (MPC) to try to achieve this goal. 
However, as noted by~\citet{Kearns18}, the individual information that MPC tries to protect can still be inferred from the learned model.
Further, the method of \citet{pmlr-v80-kilbertus18a} is limited to using demographic parity as the fairness criteria. 
}

%and achieving good accuracy.
A more recent work of~\citet{Kearns18} explored preserving differential privacy~\citep{Dwork06} while 
%at the same time of preserving 
{maintaining} 
fairness constraints. 
The authors proposed two methods:
one adds Laplace noise to training data and apply the post-processing method in~\citet{Hardt2016},
while \FINALCHANGE{another}{the other} modifies the method in~\citet{reduction} using the exponential mechanism as well as Laplace noise.
Our work differs from them in three major ways:
\begin{enumerate}[itemsep=0pt,topsep=0pt,label=(\emph{\arabic*})]
    % \item \AKMEDIT{our work can leverage \emph{any} algorithm for achieving fairness, while~\citet{Kearns18} is tied to specific algorithms};
    % %rather than modifying specific algorithms, our work can be used before applying a large group of fair algorithms;
    
    \item \FINALCHANGE{our work allows for fair classification to be done using a %vast
{\emph{any}} fairness-aware classifier, whereas the method of \citet{Kearns18} %forces
{requires the use of} a particular classifier.}{our work allows for fair classification to be done using %vast
{\emph{any}} \emph{in-process} fairness-aware classifier that allows user to specify desired fairness level. On the other hand, the first method of \citet{Kearns18} %forces
requires the use of a post-processing algorithm 
%(in-processing algorithms generally result in better trade-offs than post-processing as shown in \citet{reduction}), 
(which generally have worse trade-offs than in-processing algorithms~\citet{reduction}), 
while the second method requires the use of a single \emph{particular} classifier.}
    
    % \item although our framework can also be used for preserving differential privacy, we mainly focus on the case of data corruption  under the framework of MC learning rather than privacy;
    
    \item our focus is on designing fair-classifiers with noise-corrupted sensitive attributes; {by contrast, the main concern in~\citet{Kearns18} is achieving differential privacy}\FINALCHANGE{}{and thus they do not discuss how to deal with noise that is already present in the dataset}.
    
    \item \FINALCHANGE{we deal with not only equalized odds, but also demographic parity.}{our method is shown to work for a large class of different fairness definitions.}
\end{enumerate}

\FINALCHANGE{}{Finally, a concurrent work of~\citet{fairlearning_withprivatedata} 
builds upon our method
for the problem of preserving privacy of the sensitive attribute.
The authors use a randomized response procedure on the sensitive attribute values, followed by a two-step procedure to train a fair classifier using the processed data. 
Theoretically, their method improves upon the sample complexity of our method and extends our privacy result to the case of non-binary groups. 
However, their method solely focuses on preserving privacy rather than the general problem of sensitive attribute noise.}
%Furthermore, no empirical result has been shown for the effectiveness of their proposed method.}

% Note that while other methods, such as those described in \citet{Kearns18}, 
% may be better suited if differential privacy is the main concern, our method differs in two important ways. First, it allows for fair classification to be done using a %vast
% {broader} class of fairness-aware classifiers, whereas the method of \citet{Kearns18} %forces
% {restricts} the user to use a particular classifier.
% Second, {unlike~\citet{Kearns18}, our focus is on designing fair-classifiers with noise corrupted sensitive attributes.}

%it is important to keep in mind that the method of \citet{Kearns18} is specifically geared towards this problem, while our method can also be used to achieve fair classification using naturally noisy data.


==> Fairness under corruption NeurIPS 2019 (2)/noise_on_ay.tex <==
%auto-ignore
\subsection{Noise model}

We consider class-conditional label noise (CCN learning)\cite{Angluin88}.
Specifically, let $\rho_a^+, \rho_a^-, \rho_y^+, \rho_y^-\in [0,1]$.
We assume samples with $A=1$ flipped with probability $\rho_a^+$ and samples with $A=0$ flipped with probability $\rho_a^-$.
We also assume samples with $Y=1$ flipped with probability $\rho_y^+$ and samples with $Y=0$ flipped with probability $\rho_y^-$.
Thus, we have:
\begin{equation}
    \begin{aligned}
        \eta_a     &= (1-\rho^+_a) \cdot \eta_a + \rho^-_a \cdot (1-\eta_a)\\
        (1-\eta_a) &= \rho^+_a \cdot \eta_a + (1-\rho^-_a) \cdot (1-\eta_a)\\
        \eta_y     &= (1-\rho^+_y) \cdot \eta_y + \rho^-_y \cdot (1-\eta_y)\\
        (1-\eta_y) &= \rho^+_y \cdot \eta_y + (1-\rho^-_y) \cdot (1-\eta_y)\\
    \end{aligned}
\end{equation}

Since CCN setting is a special case of MC learning \cite{corruption}, the above setting is equivalent to the conditional probability caused by the corruption on the sensitive attribute as in 2.1 (we use the notation $\pi_{a,\cdot,\text{corr}_{ay}}$ for the corrupted base rate in this setting), and the following conditional distribution caused by the corruption on the label:
\begin{equation}
    \begin{aligned}
        &D_{\cdot,1,\text{corr}_{ay}} = (1-\alpha_y) \cdot D_{\cdot,1} + \alpha_y \cdot D_{\cdot,0}\\
        &D_{\cdot,0,\text{corr}_{ay}} = \beta_y \cdot D_{\cdot,1} + (1-\beta_y) \cdot D_{\cdot,0},
    \end{aligned}
\end{equation}
which has the corrupted base rate $\pi_{\cdot,y,\text{corr}_{ay}}$.

As shown in \citet[Appendix C]{corruption}, the parameters are as the follows:
\begin{align*}
    \pi_{a,\cdot,\text{corr}_{ay}} &= (1-\rho_a^+)\pi_{a,\cdot}+\rho_a^-(1-\pi_{a,\cdot})\\
    \alpha_a &= \pi_{a,\cdot,\text{corr}_{ay}}^{-1}(1-\pi_{a,\cdot})\rho_a^-\\
    \beta_a &= (1-\pi_{a,\cdot,\text{corr}_{ay}})^{-1}\pi_{a,\cdot}\rho_a^+\\
    \pi_{\cdot,y,\text{corr}_{ay}} &= (1-\rho_y^+)\pi_{\cdot,y}+\rho_y^-(1-\pi_{\cdot,y})\\
    \alpha_y &= \pi_{\cdot,y,\text{corr}_{ay}}^{-1}(1-\pi_{\cdot,y})\rho_y^-\\
    \beta_y &= (1-\pi_{\cdot,y,\text{corr}_{ay}})^{-1}\pi_{\cdot,y}\rho_y^+
\end{align*}




%
\subsection{Demographic Parity(To be fixed)}

\begin{theorem}\label{thm: sensitive and label noise reduction}
    Under the noise setting of section \ref{section:bothnoise}, in the DP case, the constrained optimization problem
    \begin{align*}
        \min_{f\in \mathcal{F}}& \ \ \mathrm{BER}_y^D(f)\\
        \text{s.t.}& \ \ \left| \mathbb{P}^+_{D_{0,\cdot}}(f)-\mathbb{P}^+_{D_{1,\cdot}}(f) \right| \leq \tau
    \end{align*}
    is equivalent to
    \begin{align*}
        \min_{f\in \mathcal{F}}& \ \ (1-\alpha_y-\beta_y)^{-1} \mathrm{BER}_y^{D_{\text{corr}_{ay}}}(f)\\
        \text{s.t.}& \ \ \left| \mathbb{P}^+_{D_{0,\cdot,{\text{corr}_{ay}}}}(f)-\mathbb{P}^+_{D_{1,\cdot,{\text{corr}_{ay}}}}(f) \right| \leq \tau(1-\alpha_a-\beta_a)
    \end{align*}
    
\end{theorem}
\begin{proof}[Proof]
 We know from \cite{corruption} that $\frac{1}{(1-\alpha_a - \beta_a)} \paren{\mathrm{BER}_y^{D_{\text{corr}_{ay}}}(f) - \frac{\alpha_a+\beta_a}{2}} =  \mathrm{BER}_y^D(f)$. So
 \begin{align*}
    &\min_{f\in \mathcal{F}} \ \ \mathrm{BER}_y^D(f)\\
    &\iff \min_{f\in \mathcal{F}} \ \ \frac{1}{(1-\alpha_a - \beta_a)} \paren{\BER_y^{D_{\text{corr}_{ay}}}(f) - \frac{\alpha_a+\beta_a}{2}}\\
    &\iff \min_{f\in \mathcal{F}} \frac{1}{(1-\alpha_a - \beta_a)} \BER_y^{D_{\text{corr}_{ay}}}(f)
 \end{align*}
Because the two noises are independent with each other, the constraint comes directly from \ref{thm: sensitive noise reduction}.
\end{proof}


%
\subsection{Equality of Opportunity}


==> Fairness under corruption NeurIPS 2019 (2)/problem_formulation.tex <==
%auto-ignore
\subsection{Further notation}

We denote the conditional probabilities by:
\begin{align*}
\eta_y(x)&:=\mathbb{P}[Y=1|X=x]\\
\eta_a(x)&:=\mathbb{P}[A=1|X=x]
\end{align*}

And we use the following abbreviations for simplicity:
\begin{align*}
    \mathbb{P}_{D}&:=\mathbb{P}_{(x,a,y)\sim D}\\
    \mathbb{P}^+_D(f) &:= \mathbb{P}_{D}[\sign(f(x))=1]\\
    \mathbb{P}^-_D(f) &:= \mathbb{P}_{D}[\sign(f(x))=0]
\end{align*}

Finally we denote the base rates by:
\begin{align*}
\pi_{\cdot,y}&:=\mathbb{P}[Y=1]\\
\pi_{a,\cdot}&:=\mathbb{P}[A=1]\\
\pi_{a,y}&:=\mathbb{P}[A=1,Y=1]
\end{align*}


==> Fairness under corruption NeurIPS 2019 (2)/related.tex <==
%auto-ignore
We review relevant literature on fair and noise-tolerant %, and privacy-preserving
machine learning.

%
\subsection{Fair machine learning}
\label{sec:bg-fairness}

Algorithmic fairness has gained significant attention recently because of the undesirable social impact caused by bias in machine learning algorithms~\citep{COMPAS,gendershades,Lahoti}.
There are two central %problems:
{objectives}:
%what is an appropriate fairness definition, and
%how to optimize the original objective while satisfying the chosen fairness definition.
% \EDIT{designing appropriate application-specific fairness criterion, and
% how to develop predictors that respect the chosen fairness conditions}.
designing appropriate application-specific fairness criterion, and
developing predictors that respect the chosen fairness conditions.

%To deal with the first problem, multiple fairness definitions have been proposed.
%\aditya{US English: categorized}
{Broadly, fairness objectives can be categorised} into
%These fall into two main categories: 
individual- and group-level fairness.
Individual-level fairness~\citep{Dwork:2011,Kusner,Kim} requires the treatment of ``similar'' individuals to be similar.
Group-level fairness 
asks the treatment of the groups divided based on some sensitive attributes (e.g., gender, race) to be similar.
Popular notions of group-level fairness include
demographic parity~\citep{Calders}
and
equality of opportunity~\citep{Hardt2016}%
%, and disparate mistreatment~\citep{ZafarWWW}
;
see \S\ref{section:fairnessdef} for formal definitions. 

% \EDIT{Group-level fairness criteria tend to be more conducive to algorithmic design and analysis, and is achieved by three possible ways:}
%\aditya{Don't want to say ``more conducive''. Someone working on individual fairness could get irate.}
{Group-level fairness criteria have been the subject of significant algorithmic design and analysis,}
and are achieved in three possible ways:
%
%There are three main types of method
%to achieve fairness while optimizing the original objective:
\begin{itemize}[itemsep=0pt,topsep=0pt,leftmargin=16pt]
    \item[--] pre-processing methods~\citep{ZemelICML,ZemelICLR,Lum,Johndrow:2017,Calmon:2017,delBarrio:2018,Adler:2018},
    which
    %usually embed the representation of data into a new space such that the bias is removed.
    {usually find a new representation of the data where the bias with respect to the sensitive feature is explicitly removed.}
    
    \item[--] methods enforcing fairness during training~\citep{Calders,Woodworth,ZafarWWW,reduction},
    which
    usually add a constraint that is a proxy of the fairness criteria or add a regularization term to penalise fairness violation.

    \item[--] post-processing methods~\citep{Feldman,Hardt2016},
    which usually apply a thresholding function to make the prediction satisfying the chosen fairness notion across groups.
\end{itemize}


%
\subsection{Noise-tolerant classification}

Designing noise-tolerant classifiers is a classic topic of study, concerned with the setting where one's training labels are corrupted in some manner.
Typically, works in this area postulate a particular model of label noise, and study the viability of learning under this model.
% Prominent noise models include
% symmetric and class-conditional noise~\citep{Angluin88,Bylander:1994,Blum:1996,Blum:1998},
% constant-partition noise~\citep{Decatur:1997,Ralaivola:2006},
% and instance-dependent noise~\citep{Awasthi:2015}.
% It has also been shown that learning performance degrades as label noise increases~\citep{Nettleton2010}.
Class-conditional noise (CCN)~\citep{Angluin88} is one such %well-studied 
{effective}
noise model.
Here, samples from each class have their labels flipped with some constant (but class-specific) probability.
Algorithms that deal with CCN corruption have been well studied~\citep{natarajan2013learningw,Liu2016ClassificationWN,northcutt2017rankpruning}.
These methods typically first estimate the noise rates, which are then used for prediction.
A special case of CCN learning is learning from positive and unlabelled data (PU learning)~\citep{Elkan},
where in lieu of explicit negative samples, one has a pool of unlabelled data.

%Multiple noise settings have been explored, e.g., mutually contaminated (MC) learning~\citep{Scott13} and class-conditional noise (CCN) learning~\citep{Angluin88}.
\iffalse
Our particular interest in this paper will be in the class-conditional noise (CCN) setting.
Here, samples from each class have their labels flipped with some constant (but class-specific) probability.
Algorithms that deal with CCN corruption have been well studied~\citep{natarajan2013learningw,Liu2016ClassificationWN,northcutt2017rankpruning}.
These methods typically first estimate the noise rates and then use these rates for prediction.
The CCN model is a special case of the more general mutually contaminated (MC) learning model~\citep{Scott13}.

An important related problem is that of learning from positive and unlabelled data (PU learning)~\citep{Denis:1998a},
where in lieu of explicit negative samples, one has a pool of unlabelled data.
PU learning in turn has two prominent settings:
the censoring setting, which is a special case of class-conditional noise~\citep{Elkan}, and
the case-controlled setting~\citep{Ward:2009}, which is a special case of class-conditional noise \emph{plus} an additional rebalancing of labels.
Both of these can be modelled as a special case of a more general corrupted label framework~\citep{pmlr-v30-Scott13,corruption}.
\fi

% PU learning in turn has two prominent settings.
% In the censoring setting of the problem~\citep{Elkan}, one imagines first drawing labelled samples, and then placing some fraction of positives in the unlabelled pool.
% In the case-controlled setting~\citep{Ward:2009}, one imagines independently drawing samples from the positive and marginal distribution over instances.
% %Both of these can be modelled as a special case of MC learning.

Our interest in this paper will be the \emph{mutually contaminated} (MC) \emph{learning} noise model~\citep{Scott13}.
This model (described in detail in \S\ref{sec:mc-learning}) captures both CCN and %(both settings of)
PU learning as special cases~\citep{pmlr-v30-Scott13,corruption}, {as well as other interesting noise models}.



%\subsection{fair classification preserving privacy of sensitive attribute}
%\ZIYUANEDIT{There exist previous work \cite{pmlr-v80-kilbertus18a} that try to preserve privacy of every individual's sensitive attribute's value while learning a fair classifier by employing the cryptographic tool of secure multiparty computation (MPC). However, as shown in \cite{Kearns18}, the individual information that MPC tries to protect can be inferred from the learned model. Besides, their method is limited to using Demographic Parity as fairness creteria.}
%\ZIYUANEDIT{Concurrent work \cite{fairlearning_withprivatedata} on preserving privacy of sensitive attribute uses a randomized response procedure on the sensitive attribute values and a two-step procedure to train a fair classifier using the processed data. Theoretically, their method improves the sample complexity compared with our method and extends our privacy result to the case of non-binary groups. However, their method solely focuses on preserving privacy rather than a general noise setting. Besides, no empirical result has been shown for the effectiveness of their proposed method.
%}

% %
% \subsection{Fairness and differential privacy}

% Recently,~\citet{Kearns18} explored preserving differential privacy~\citep{Dwork06} while %at the same time of preserving 
% {maintaining} fairness constraints. 
% %and achieving good accuracy.
% The authors proposed two methods:
% one adds Laplace noise to training data and apply the post-processing method in~\citet{Hardt2016},
% while another modifies the method in~\citet{reduction} using the exponential mechanism as well as Laplace noise.
% Our work differs from them in three major ways:
% \begin{enumerate*}[itemsep=0pt,topsep=0pt,label=(\emph{\arabic*})]
%     \item \AKMEDIT{our work can leverage \emph{any} algorithm for achieving fairness, while~\citet{Kearns18} is tied to specific algorithms};
%     %rather than modifying specific algorithms, our work can be used before applying a large group of fair algorithms;
%     \item although our framework can also be used for preserving differential privacy, we mainly focus on the case of data corruption  under the framework of MC learning rather than privacy;
%     \item we deal with not only equalized odds, but also demographic parity.
% \end{enumerate*}


==> experiment_sanity_check.tex <==
%auto-ignore
\iffalse




% \subsubsection{Assuming we know noise rates}
% \label{ssec:num1:known_nr}

Following a large number of previous studies,
we use four datasets for our experiments:
\begin{itemize}[itemsep=0pt,topsep=0pt]
    \item {\tt adult}, a dataset from the UCI repository~\citep{UCI}.
    The task is to predict if one's annual income is more than 50k and the sensitive attribute is gender or race. 
    The data comprises 48842 examples and 14 features.

    \item {\tt german}, another dataset from the UCI repository~\citep{UCI}. The task is to predict if one has good credit and the sensitive attribute is if a person is foreign.
    The data comprises 1000 examples and 20 features.
    
    \item {\tt Law School}, a dataset from LSAC~\citep{Wightman}.
    The task is to predict the passage of the bar exam and the sensitive attribute is race. 
    The data comprises 16638 examples and 11 features.
    
    \item {\tt COMPAS}, a dataset from Propublica~\citep{COMPAS}.
    The task is to predict recidivism and the sensitive attribute is race.
    The data comprises 7918 examples and 10 features.
    

\end{itemize}

We now present experiments in several progressively challenging settings:
where there is noise in $A$,
and where the noise aims to preserve privacy.


%
\subsection{Noise in the sensitive attribute}

For simplicity, we add noise according to CCN model, i.e. we randomly flip the sensitive attribute of samples with $A = 1$ with probability $\rho^+$ and randomly flip the sensitive attribute of samples with $A = 0$ with probability $\rho^-$.
For further simplicity, we let $\rho:=\rho^+=\rho^-$.

We present results first assuming prior knowledge of the noise rates,
and then where the noise rates are estimated from data.


%
% \subsubsection{Assuming we know noise rates}
% \label{ssec:num1:known_nr}

We assume that we know the values of $\rho$. In this case, we can estimate $\alpha$ and $\beta$ using relationship specified in 3.3.2.

As a baseline (termed {\sf denoise}) and then apply \cite{reduction}. We apply the {\sf RankPrune} method in \cite{northcutt2017rankpruning} to denoise $A$. {\sf denoise} is a two-steps method, it first estimate noise rates and then estimate A based on the estimated noise rates. For the purpose of fair comparison, we pass the known noise rates to {\sf denoise} and only use its second step in this section.

Our method (termed {\sf cor\_scale}) scales the input parameter $\tau$ and then ~\citet{reduction} to perform fair classification.

We run experiments at noise level $\rho=0.2$ on both {\tt adult} and {\tt COMPAS}.

We compare the relationship between the input $\epsilon$ and training/testing error/fairness violation under both DP and EO of four situations.

\begin{itemize}
    \item Apply \cite{reduction} on no-corrupted data(termed {\sf nocor}).
    \item Apply \cite{reduction} on corrupted data(termed {\sf cor}).
    \item {\sf denoise}
    \item {\sf cor scale}
\end{itemize}

Each plot is the average of three runs. At each run, we make a random $80$--$20$ train-test split.

The $x$-axis is the given input $\tau$ that controls the strictness of fairness constraint and $y$-axis is DEO or DDP as defined in \ref{section:fairnessdef}.

It can be seen from Figures~\ref{fig:DP_compas_known} and \ref{fig:EO_compas_known} that the fairness violation and error rates of {\sf cor\_scale} are much closer to {\sf no\_cor} when compared with both {\sf cor} and {\sf denoise} under both DP and EO.

This result is consistent with our derivation and implies that our scaling indeed helps to achieve the originally wanted degree of fairness before corruption.
Besides, without surprise, due to down-scaling the $\epsilon$, the corruption with scaling causes slightly higher error than the {\sf no\_cor} for both datasets on both training set and testing set.

See Appendix \ref{appendix:knowing-nr-training} for the corresponding results on the training set.

See Appendix \ref{appendix:noise-level} for the same experiment performed at different noise levels.
\fi




\iffalse
\subsubsection{Assuming we do not know noise rates}

We next turn to the more realistic (but challenging) setting where the noise rates are unknown.
Here, as a baseline (termed {\sf denoise}), we apply the {\sf RankPrune} method in \cite{northcutt2017rankpruning} to denoise $A$, and then apply \cite{reduction}.
Our method (termed {\sf scale\_est}) follows Algorithm~\ref{alg:reduction},
employing {\sf RankPrune} to estimate $\rho^+$ and $\rho^-$ (and thus $\hat{\alpha}_a$ and $\hat{\beta}_a$),
and then ~\citet{reduction} to perform fair classification.

We use the same setup as before (except choosing $\rho=0.3$ to see clearer pattern). We compare the training/testing fairness violation/error rate of the two methods at different input $\epsilon$. For the purpose of comparison, we also include the three curves specified in the previous section.

It can be seen from Figure~\ref{fig:DP_compas_five} that our method produces better preservation of fairness requirement compared with the baseline method.

\begin{center}
    \includegraphics[width=0.4\textwidth]{imgs2/DP_Agarwal_compas_03_3_ref_five}
    \captionof{figure}{(DP) Relationship between input epsilon and fairness violation/error on the UCI {\tt adult} dataset.}
    \label{fig:DP_compas_five}
\end{center}
\fi

==> noise_on_ay.tex <==
%auto-ignore
\subsection{Noise model}

We consider class-conditional label noise (CCN learning)\cite{Angluin88}.
Specifically, let $\rho_a^+, \rho_a^-, \rho_y^+, \rho_y^-\in [0,1]$.
We assume samples with $A=1$ flipped with probability $\rho_a^+$ and samples with $A=0$ flipped with probability $\rho_a^-$.
We also assume samples with $Y=1$ flipped with probability $\rho_y^+$ and samples with $Y=0$ flipped with probability $\rho_y^-$.
Thus, we have:
\begin{equation}
    \begin{aligned}
        \eta_a     &= (1-\rho^+_a) \cdot \eta_a + \rho^-_a \cdot (1-\eta_a)\\
        (1-\eta_a) &= \rho^+_a \cdot \eta_a + (1-\rho^-_a) \cdot (1-\eta_a)\\
        \eta_y     &= (1-\rho^+_y) \cdot \eta_y + \rho^-_y \cdot (1-\eta_y)\\
        (1-\eta_y) &= \rho^+_y \cdot \eta_y + (1-\rho^-_y) \cdot (1-\eta_y)\\
    \end{aligned}
\end{equation}

Since CCN setting is a special case of MC learning \cite{corruption}, the above setting is equivalent to the conditional probability caused by the corruption on the sensitive attribute as in 2.1 (we use the notation $\pi_{a,\cdot,\text{corr}_{ay}}$ for the corrupted base rate in this setting), and the following conditional distribution caused by the corruption on the label:
\begin{equation}
    \begin{aligned}
        &D_{\cdot,1,\text{corr}_{ay}} = (1-\alpha_y) \cdot D_{\cdot,1} + \alpha_y \cdot D_{\cdot,0}\\
        &D_{\cdot,0,\text{corr}_{ay}} = \beta_y \cdot D_{\cdot,1} + (1-\beta_y) \cdot D_{\cdot,0},
    \end{aligned}
\end{equation}
which has the corrupted base rate $\pi_{\cdot,y,\text{corr}_{ay}}$.

As shown in \citet[Appendix C]{corruption}, the parameters are as the follows:
\begin{align*}
    \pi_{a,\cdot,\text{corr}_{ay}} &= (1-\rho_a^+)\pi_{a,\cdot}+\rho_a^-(1-\pi_{a,\cdot})\\
    \alpha_a &= \pi_{a,\cdot,\text{corr}_{ay}}^{-1}(1-\pi_{a,\cdot})\rho_a^-\\
    \beta_a &= (1-\pi_{a,\cdot,\text{corr}_{ay}})^{-1}\pi_{a,\cdot}\rho_a^+\\
    \pi_{\cdot,y,\text{corr}_{ay}} &= (1-\rho_y^+)\pi_{\cdot,y}+\rho_y^-(1-\pi_{\cdot,y})\\
    \alpha_y &= \pi_{\cdot,y,\text{corr}_{ay}}^{-1}(1-\pi_{\cdot,y})\rho_y^-\\
    \beta_y &= (1-\pi_{\cdot,y,\text{corr}_{ay}})^{-1}\pi_{\cdot,y}\rho_y^+
\end{align*}




%
\subsection{Demographic Parity(To be fixed)}

\begin{theorem}\label{thm: sensitive and label noise reduction}
    Under the noise setting of section \ref{section:bothnoise}, in the DP case, the constrained optimization problem
    \begin{align*}
        \min_{f\in \mathcal{F}}& \ \ \mathrm{BER}_y^D(f)\\
        \text{s.t.}& \ \ \left| \mathbb{P}^+_{D_{0,\cdot}}(f)-\mathbb{P}^+_{D_{1,\cdot}}(f) \right| \leq \tau
    \end{align*}
    is equivalent to
    \begin{align*}
        \min_{f\in \mathcal{F}}& \ \ (1-\alpha_y-\beta_y)^{-1} \mathrm{BER}_y^{D_{\text{corr}_{ay}}}(f)\\
        \text{s.t.}& \ \ \left| \mathbb{P}^+_{D_{0,\cdot,{\text{corr}_{ay}}}}(f)-\mathbb{P}^+_{D_{1,\cdot,{\text{corr}_{ay}}}}(f) \right| \leq \tau(1-\alpha_a-\beta_a)
    \end{align*}
    
\end{theorem}
\begin{proof}[Proof]
 We know from \cite{corruption} that $\frac{1}{(1-\alpha_a - \beta_a)} \paren{\mathrm{BER}_y^{D_{\text{corr}_{ay}}}(f) - \frac{\alpha_a+\beta_a}{2}} =  \mathrm{BER}_y^D(f)$. So
 \begin{align*}
    &\min_{f\in \mathcal{F}} \ \ \mathrm{BER}_y^D(f)\\
    &\iff \min_{f\in \mathcal{F}} \ \ \frac{1}{(1-\alpha_a - \beta_a)} \paren{\BER_y^{D_{\text{corr}_{ay}}}(f) - \frac{\alpha_a+\beta_a}{2}}\\
    &\iff \min_{f\in \mathcal{F}} \frac{1}{(1-\alpha_a - \beta_a)} \BER_y^{D_{\text{corr}_{ay}}}(f)
 \end{align*}
Because the two noises are independent with each other, the constraint comes directly from \ref{thm: sensitive noise reduction}.
\end{proof}


%
\subsection{Equality of Opportunity}


==> problem_formulation.tex <==
%auto-ignore
\subsection{Further notation}

We denote the conditional probabilities by:
\begin{align*}
\eta_y(x)&:=\mathbb{P}[Y=1|X=x]\\
\eta_a(x)&:=\mathbb{P}[A=1|X=x]
\end{align*}

And we use the following abbreviations for simplicity:
\begin{align*}
    \mathbb{P}_{D}&:=\mathbb{P}_{(x,a,y)\sim D}\\
    \mathbb{P}^+_D(f) &:= \mathbb{P}_{D}[\sign(f(x))=1]\\
    \mathbb{P}^-_D(f) &:= \mathbb{P}_{D}[\sign(f(x))=0]
\end{align*}

Finally we denote the base rates by:
\begin{align*}
\pi_{\cdot,y}&:=\mathbb{P}[Y=1]\\
\pi_{a,\cdot}&:=\mathbb{P}[A=1]\\
\pi_{a,y}&:=\mathbb{P}[A=1,Y=1]
\end{align*}

